A Self-Supervised Approach to Reconstruction in Sparse X-Ray Computed Tomography

Computed tomography has propelled scientific advances in fields from biology to materials science. This technology allows for the elucidation of 3-dimensional internal structure by the attenuation of x-rays through an object at different rotations relative to the beam. By imaging 2-dimensional projections, a 3-dimensional object can be reconstructed through a computational algorithm. Imaging at a greater number of rotation angles allows for improved reconstruction. However, taking more measurements increases the x-ray dose and may cause sample damage. Deep neural networks have been used to transform sparse 2-D projection measurements to a 3-D reconstruction by training on a dataset of known similar objects. However, obtaining high-quality object reconstructions for the training dataset requires high x-ray dose measurements that can destroy or alter the specimen before imaging is complete. This becomes a chicken-and-egg problem: high-quality reconstructions cannot be generated without deep learning, and the deep neural network cannot be learned without the reconstructions. This work develops and validates a self-supervised probabilistic deep learning technique, the physics-informed variational autoencoder, to solve this problem. A dataset consisting solely of sparse projection measurements from each object is used to jointly reconstruct all objects of the set. This approach has the potential to allow visualization of fragile samples with x-ray computed tomography. We release our code for reproducing our results at: https://github.com/vganapati/CT_PVAE .

==> scraps.tex <==
With these tomograms, corresponding noisy low-dose CT measurements can be simulated through the forward model (i.e. the known physics of the imaging process). From the measurement-reconstruction pairs, a deep neural network can be trained to approximate the correspondence. After training, at inference, the tomogram for any low-dose measurement can be predicted by the network. However, 

This becomes a chicken-and-egg problem: high-quality reconstructions cannot be generated without deep learning, and the deep neural network cannot be learned without the reconstructions. 

The second open question concerns the capture of low-dose measurements. For fragile samples, there is a total allowable x-ray dose. By randomizing the allocation of the total dose amongst rotation angles for each sample, the  probability distribution of the objects can be inferred; this is the underlying assumption of prior work. However, understanding how to randomize is an open question. Should many angles be sampled with an extremely low dose or should fewer angles be sampled with higher dose each? This work investigates the dependence of reconstruction quality on the probability distribution that generates the dose allocation.

This project formulates a variational autoencoder trained only with $M$ to generate $P(O|M)$.
The objective is to develop a reconstruction method that can be trained in an unsupervised manner without ground truth, only with low-dose CT measurements. 

More precisely, computed tomography aims to reconstruct some object $O$ from a set of $n$ noisy measurements $M = [M_1, M_2, ..., M_n]$. 

Our probabilistic formulation of the computational imaging problem permits uncertainty quantification, in contrast to most reconstruction algorithms that only yield a point estimate. Another key difference from standard methods is our joint reconstruction of a set of objects as opposed to consideration of a single object at a time.

Deep neural networks are chosen for function approximation due to their theoretical ability to approximate any function \cite{cybenko_approximation_1989, hornik_approximation_1991, leshno_multilayer_1993} and practical success in approximating high-dimensional functions \cite{lecun_deep_2015}. 

\begin{figure}[h]
%\vspace{0em}
\centering
\includegraphics[width=0.55\textwidth]{figures/regular_generator.png}
\caption{\emph{Generating object $O$ from a latent variable $z$.}}
%\vspace{0em}
\label{fig:gen}
\end{figure}


Deep neural networks are chosen for function approximation due to their theoretical ability to approximate any function \cite{cybenko_approximation_1989, hornik_approximation_1991, leshno_multilayer_1993} and practical success in approximating high-dimensional functions \cite{lecun_deep_2015}. 

The latent space of the generative network can then be optimized iteratively to reconstruct a desired measurement.
These object reconstructions can be used to create training pairs for a deep neural network. Alternatively,
This method is used to create a neural network prior for iterative optimization in 
